A Sequential Quadratic Programming Approach to the Solution of Open-Loop Generalized Nash Equilibria for Autonomous Racing

Dynamic games can be an effective approach for modeling interactive behavior between multiple competitive agents in autonomous racing and they provide a theoretical framework for simultaneous prediction and control in such scenarios. In this work, we propose DG-SQP, a numerical method for the solution of local generalized Nash equilibria (GNE) for open-loop general-sum dynamic games for agents with nonlinear dynamics and constraints. In particular, we formulate a sequential quadratic programming (SQP) approach which requires only the solution of a single convex quadratic program at each iteration. The three key elements of the method are a non-monotonic line search for solving the associated KKT equations, a merit function to handle zero sum costs, and a decaying regularization scheme for SQP step selection. We show that our method achieves linear convergence in the neighborhood of local GNE and demonstrate the effectiveness of the approach in the context of head-to-head car racing, where we show significant improvement in solver success rate when comparing against the state-of-the-art PATH solver for dynamic games. An implementation of our solver can be found at https://github.com/zhu-edward/DGSQP.

==> results.tex <==
\section{Results} \label{sec:results}

We now present the results of learning a game-theoretic value function and its application in closed-loop with a racing MPC policy. In the following, the game-theoretic value function $V_{GT}$ is modeled as an MLP with two hidden layers of size 48 and \texttt{tanh} activation function. Training is done on datasets of $\sim$1800 GNE solutions from joint initial conditions that were sampled from the L-shaped track in Figure~\ref{fig:exemplary_gnes}. We use the Adam optimizer with scheduled learning rate and stop training if no improvement is observed after 10 epochs.

\subsection{Open-Loop Results}



\subsection{Closed-Loop Head-to-Head Racing Formulation}

In the following sections, we examine the performance of our learned game-theoretic value function when incorporated into the following raceline-tracking finite-horizon optimal control problem for head-to-head racing:
\begin{subequations} \label{eq:racing_optimal_control_problem}
    \begin{align}
         \min_{\mathbf{u}} \ & \ \sum_{t=0}^{N-1} \|x_t-\bar{x}_{k+t}\|_Q^2 + \|u_t\|_{R_1}^2 + \|\Delta u_t\|_{R_2}^2 \nonumber \\
         & \qquad \qquad \qquad \qquad + V_{GT}(x_N, \hat{x}_{k+N}) \label{eq:racing_cost} \\
         \text{subject to} \ & \ x_0 = x_k, \label{eq:racing_initial_condition}\\
         & \ x_{t+1} = f(x_t, u_t), \label{eq:racing_dynamics}\\
         & \ x_l \leq x_t \leq x_u, \label{eq:racing_state_bounds}\\
         & \ u_l \leq u_t \leq u_u, \ \Delta u_l \leq \Delta u_t \leq \Delta u_u, \label{eq:racing_input_bounds}\\
         & \|p(x_t) - \hat{p}_{k+t}\|_2^2 \geq (r+\hat{r}_{k+t})^2, \label{eq:racing_collision_avoidance}\\
         & a^f(x_t,u_t), a^r(x_t,u_t) \leq \mu g. \label{eq:racing_friction_circle}
    \end{align}
\end{subequations}
We denote the solution to \eqref{eq:racing_optimal_control_problem} as $\mathbf{u}_k^{\star}(x_k, \bar{\mathbf{x}}_k, \hat{\mathbf{z}}_k)$ which, at time step $k$, is a function of the ego state $x_k$, the raceline $\bar{\mathbf{x}}_k$, and the prediction of the opponent $\hat{\mathbf{z}}_k$, where $\hat{z}_{k+t} = (\hat{x}_{k+t}, \hat{r}_{k+t})$ denotes a nominal state and collision buffer radius of the opponent at time step $k+t$. The stage costs in \eqref{eq:racing_cost} are comprised of tracking, input, and input rate penalties with $Q, R_1, R_2 \succeq 0$, and the learned game-theoretic value function $V_{GT}$ as the terminal cost. \eqref{eq:racing_initial_condition} and \eqref{eq:racing_dynamics} are the initial condition and dynamics constraints respectively, where we use the Frenet frame dynamic bicycle model with Pacejka tire model as discussed in Section~\ref{sec:approximation} for $f$. \eqref{eq:racing_state_bounds} and \eqref{eq:racing_input_bounds} are simple bounds on the vehicle state and inputs, which are used to impose track boundary, actuator saturation, and actuator rate constraints. \eqref{eq:racing_collision_avoidance} is the collision avoidance constraint given an opponent prediction with nominal position $\hat{p}_{k+t}$ and collision buffer radius $\hat{r}_{k+t}$. Finally, \eqref{eq:racing_friction_circle} are friction circle constraints on the front and rear tires for the tire-road friction coefficient $\mu$. Here, $a^f$ and $a^r$ are functions which return the magnitude of the acceleration experienced by the front and rear tires respectively given the state and input at stage $t$. In typical receding horizon fashion, our racing policy applies the first element of $\mathbf{u}_k^\star$ at time $k$, then resolves \eqref{eq:racing_optimal_control_problem} at the next time step. We note that since our goal is to demonstrate the impact of the value function, for simplicity, we generate $\hat{\mathbf{z}}_k$ using an oracle but corrupt it with Gaussian noise. We use time-varying collision buffer radii, i.e. $\hat{r}_k < \hat{r}_{k+1} < \dots < \hat{r}_{k+N}$, to capture robustness against growing prediction uncertainty. Of course, this could be replaced by any number of existing trajectory prediction schemes, though we defer an investigation of their impact on racing performance to future work.

In the following simulation and hardware races, we denote the vehicle using \eqref{eq:racing_optimal_control_problem} as GT and we compare against a non-game-theoretic optimal control policy which is identical to \eqref{eq:racing_optimal_control_problem} in all but the terminal cost function. Namely, we replace $V_{GT}$ with a maximum progress value function $V_{MP}(x, \hat{x}) = s(\hat{x})-s(x)$. Of course, since the opponent prediction is treated as a parameter in \eqref{eq:racing_optimal_control_problem}, $s(\hat{x})$ is a constant and therefore has no effect on the optimal solution. However, we keep the value function in this form in order to make a direct comparison to $V_{GT}$, which, as described in Section~\ref{sec:value_function_learning}, predicts the progress advantage of the ego vehicle against its opponent. We denote the vehicle using this baseline as MP. Finally, we define an optimal control problem which removes the terminal cost in \eqref{eq:racing_cost} and the collision avoidance constraint \eqref{eq:racing_collision_avoidance} from \eqref{eq:racing_optimal_control_problem}. This simple raceline-tracking policy is used when the cars are not interacting with each other (i.e. $>$3 car lengths apart).

All races are initialized with the two cars outside of our defined interaction range. While both vehicles track precomputed racelines of the same shape (i.e. the red line in Figure~\ref{fig:exp_attack}), similar to \cite{schwarting2021stochastic} and \cite{wang2019gameb}, we force the initially leading car to be slower than the initially trailing car by reducing its velocity profile by 10\%. In the remainder, we call these two cars slow and fast respectively. When the vehicles come within the 3 car length threshold, they switch to either the GT or MP policies. If the trailing car overtakes the leading car, then both cars switch to the raceline-tracking policy for the remainder of the race. The race ends after 3 full laps are completed by both cars. Finally, we formulate both the GT and MP optimal control problems using CasADi \cite{Andersson2019} with a horizon length of $N=10$ and discretization step of $\Delta t = 0.1$s. These are solved using real-time iteration with the QP solver HPIPM \cite{frison2020hpipm}. 

\subsection{Simulation Monte-Carlo Experiment}

\begin{figure}[t] 
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/sim_race_outcomes.png}
    \vspace{-0.5cm}
    \caption{Histogram of the lead (in number of car lengths) of the faster agent over the slower agent at the end of the simulation races. Green bars indicate races where the faster agent wins, red bars indicate losses. The black dashed line indicates the average lead over all trials.}
    \label{fig:sim_race_outcomes}
\end{figure}

For our simulation study, we sample 100 joint initial conditions from a precomputed raceline for the L-shaped track such that the two cars begin with a difference in track progress of 2m. For each initial condition, four scenarios are simulated. Namely, Fast GT vs. Slow GT, Fast GT vs Slow MP, Fast MP vs. Slow GT, and Fast MP vs. Slow MP, which indicate the assignment of the aforementioned MPC policies to each of the two cars. The outcomes of the races are summarized in Figure~\ref{fig:sim_race_outcomes}. From the results, we first note that when using GT, the faster car is able to win all races. However, there is a clear reduction in its average lead at the end of the race when the slower car also uses GT, which indicates that GT allows the slower car to defend its position more effectively than MP by leveraging the game-theoretic value function. This is further emphasized in the case of Fast MP vs. Slow GT where the slower car is able to successfully defend its lead and win all races with the game-theoretic MPC policy. We include results from the Fast MP vs. Slow MP scenario as a baseline to show that when no game-theoretic component is included, the faster car has a win rate of approximately 50\%. From these results, it is clear that the learned game-theoretic value function imparts a clear competitive advantage in both overtaking and position defense scenarios. Next, we will show this in detail through our hardware experiments.

% \begin{figure*}[t] 
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/sim_attack_compare_fast.png}
%     \caption{\textbf{(Top)} The faster (blue) car with MP is unable to overtake the slower (green) car with GT. \textbf{(Bottom)} The faster car with GT is able to overtake the slower car with GT. The heatmaps and black level curves visualize the value functions used in this scenario by the faster (blue) car.}
%     \label{fig:sim_attack}
% \end{figure*}

% \begin{figure*}[t] 
%     \centering
%     \includegraphics[width=0.99\linewidth]{figures/sim_defense_compare_slow.png}
%     \caption{\textbf{(Top)} The slower (green) car with MP is unable to defend its position against the faster (blue) car with GT. \textbf{(Bottom)} The slower car with GT is able to defend its position against the faster car with GT. The heatmaps and black level curves visualize the value functions used in this scenario by the slower (green) car.}
%     \label{fig:sim_defense}
% \end{figure*}

% \begin{figure*}[t] 
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/sim_attack_compare.png}
%     \caption{\textbf{(Top)} The faster car with MP is unable to successfully attack and overtake the slower car with GT. a) and b) visualize the value functions used in this scenario by the faster and slower cars respectively. \textbf{(Bottom)} The faster car with GT is able to successfully attack and overtake the slower car with GT. c) and d) visualize the value functions used in this scenario by the faster and slower cars respectively}
%     \label{fig:sim_attack}
% \end{figure*}

% \begin{figure*}[t] 
%     \centering
%     \includegraphics[width=0.99\linewidth]{figures/sim_defense_compare.png}
%     \caption{\textbf{(Top)} The slower car with MP is unable to successfully defend its position against faster car with GT. a) and b) visualize the value functions used in this scenario by the faster and slower cars respectively. \textbf{(Bottom)} The slower car with GT is able to successfully defend its position against the faster car with GT. c) and d) visualize the value functions used in this scenario by the faster and slower cars respectively}
%     \label{fig:sim_defense}
% \end{figure*}

\subsection{Hardware Experiments}

\begin{table}[t]
\centering
\caption{Outcomes of the hardware experiments}
% \vspace{-0.2cm}
\begin{tabular}{c|c|c} 
% \toprule
Scenario & Races won (fast/slow) & Avg. lead (fast) \\
\midrule[1pt]
Fast GT vs. Slow GT & 4/1 & 6.10 \\
Fast GT vs. Slow MP & 5/0 & 9.14 \\
Fast MP vs. Slow GT & 0/5 & -1.28
\end{tabular}
\label{tab:hardware_race_outcomes}
% \vspace{-0.6cm}
\end{table}

\begin{figure*}[t] 
    \centering
    \includegraphics[width=0.99\linewidth]{figures/exp_attack_compare_fast.png}
    \caption{\textbf{(Top)} The faster (blue) car with MP is unable to overtake the slower (green) car with GT. \textbf{(Bottom)} The faster car with GT is able to overtake the slower car with GT. The heatmaps and black level curves visualize the value functions used in this scenario by the faster (blue) car.}
    \label{fig:exp_attack}
\end{figure*}

\begin{figure}[t] 
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/exp_attack_lateral_position.png}
    \caption{Lateral position traces from two racing scenarios. The vertical black lines correspond to the time stamps in Figure~\ref{fig:exp_attack}.}
    \label{fig:exp_attack_lateral_position}
\end{figure}

\begin{figure*}[t] 
    \centering
    \includegraphics[width=0.8\linewidth]{figures/exp_defense_compare_slow.png}
    \caption{\textbf{(Top)} The slower (green) car with MP is unable to defend its position against the faster (blue) car with GT. \textbf{(Bottom)} The slower car with GT is able to defend its position against the faster car with GT. The heatmaps and black level curves visualize the value functions used in this scenario by the slower (green) car.}
    \label{fig:exp_defense}
\end{figure*}

\begin{figure}[t] 
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/exp_defense_friction.png}
    \caption{Traces of the number of $g$s experienced by the rear tire. The horizontal dashed line indicates the limit of friction with $\mu=0.8$. The vertical black lines correspond to the time stamps in Figure~\ref{fig:exp_defense}.}
    \label{fig:exp_defense_friction}
\end{figure}

We conducted hardware experiments on a 1/10th scale RC car platform where state feedback is provided by an OptiTrack motion capture system. The MPC policies for the two cars are both run at 10 Hz on a laptop with a 2.6 GHz 9th-Gen Intel Core i7 CPU and communication of control commands and state measurements are handled using ROS2. We pick 5 different joint initial poses for the two cars and run three racing scenarios of 4 laps from each of these starting conditions, i.e. Fast GT vs. Slow GT, Fast GT vs. Slow MP, and Fast MP vs. Slow GT. The results are summarized in Table~\ref{tab:hardware_race_outcomes}, where we can see that the outcomes of these races closely mirror those from the simulation study in both the win rates as well as the average lead of the faster car. In order to illustrate the differences between the GT and MP policies, we show two interactions in Figures~\ref{fig:exp_attack} and \ref{fig:exp_defense} where we visualize the MPC plans and value function heatmaps to highlight the differences in how the GT and MP value functions guide the short-horizon MPC solution. In particular, we will show through these two examples how our racing policy is able to leverage strategic guidance from the game-theoretic value function and to combine it with the benefits of model-based optimal control to compete at the limit of performance.

In Figure~\ref{fig:exp_attack}, we show an overtaking attempt by the faster agent and where the slower agent uses the GT policy. The top row of frames shows the scenario when the faster agent uses the MP value function. While this value function directly encourages the agent to make progress along the track, i.e. to maximize $s$, it does not provide any guidance in terms of the lateral position that the car should aim for as all points with the same $s$ coordinate are of equal value. On the other hand, when the faster agent uses the GT value function, we can see in the bottom frames that not only does the learned value function encourage track progression, but we also observe non-linear level curves which indicate a preference for certain lateral positions for a given $s$. 
% In fact, we note that the high value regions shown in these frames match target regions in conventional racing strategy which looks to minimize the curvature of the path taken through turns, thereby allowing the agent to carry higher speed. 
The influence of the MP and GT value functions on the the faster car is highlighted in the red shaded region of Figure~\ref{fig:exp_attack_lateral_position}, where we can see a significantly larger difference in lateral position between the faster and slower cars when GT is used. By leveraging guidance from the GT value function, the faster agent is able to find an inside line through the chicane and 180\degree \ turn which forces the slower agent to deviate from its raceline in order to avoid collision. This finally results in a successful overtake by the faster agent. 

In Figure~\ref{fig:exp_defense}, we show a position defense attempt by the slower agent and where the faster agent uses the GT policy. From these frames, we see that the GT value function indicates preference for lateral track positions in the vicinity of the precomputed raceline (of which the learned value function had no prior knowledge). Moreover, in the second and third columns of Figure~\ref{fig:exp_defense}, we can clearly see from the MPC solutions for the slower agent that the GT value function causes it to speed up in order to defend its lead against the faster agent as it directly captures the value associated with the velocity states of the vehicle. Overall, these results indicate that by learning from GNE, our GT value function can automatically encode various aspects of conventional racing strategy which can then be leveraged to achieve good competitive performance against an opponent in both overtaking and position defense scenarios.
